Identifying Metric Structures of Deep Latent Variable Models

Deep latent variable models learn condensed representations of data that, hopefully, reflect the inner workings of the studied phenomena. Unfortunately, these latent representations are not statistically identifiable, meaning they cannot be uniquely determined. Domain experts, therefore, need to tread carefully when interpreting these. Current solutions limit the lack of identifiability through additional constraints on the latent variable model, e.g. by requiring labeled training data, or by restricting the expressivity of the model. We change the goal: instead of identifying the latent variables, we identify relationships between them such as meaningful distances, angles, and volumes. We prove this is feasible under very mild model conditions and without additional labeled data. We empirically demonstrate that our theory results in more reliable latent distances, offering a principled path forward in extracting trustworthy conclusions from deep latent variable models.

==> sections/introduction.tex <==
\section{Introduction}

In the context of learning useful latent representations through maximum likelihood, identifiability presents a critical problem. In statistics literature it refers to the challenge of uniquely determining a model's parameters. In representation learning this is equivalent to the existence of representations that are indistinguishable from the perspective of the marginal likelihood of observed data. While this issue may seem insignificant when focusing solely on model performance—since state-of-the-art generative models can effectively estimate the density of high-dimensional data without emphasizing the specific representations learned by underlying architectures like U-nets or Transformers \citep{lipman2022flow, sohl2015deep, ho2020denoising, rombach2022high}—its significance becomes apparent when the goal shifts to recovering representations that elucidate the mechanisms behind the data-generating process. In such cases, the lack of identifiability guarantees constitutes a major obstacle to critical applications in science and medicine as well as undermines further efforts in disentangling latent factors or estimating causal relationships.

To illustrate unidentifiability, consider a simple linear model with Gaussian distributional assumptions on both the prior over the latent variables and the conditional distribution over the observed samples. In this case, the rotational symmetry of the Gaussian distribution leads to rotational matrices making up the set of \textit{indeterminacy transformations} for the model. Under this model, when such a transformation is applied to the latent variables, the resulting marginal distribution of the data remains unchanged, thus making delineation impossible. While the set of rotational matrices is already infinite in the case of a simple model, the models of practical interest include deep latent variable models such as VAEs \citep{VAE}, where the set of indeterminacy transformations represents a potentially larger and uncharacterized infinity.

% \begin{wrapfigure}[12]{r}{0.3\textwidth}
% \vspace{-7mm}
% \centering
%         \begin{overpic}[unit=1mm,width=\linewidth]{pics/3d_gaussian_distribution.pdf}  % grid
%         \put(12,5){$Z_1$}
%         \put(31,7){$Z_2$}
%         \end{overpic}
%         \vspace{-2mm}
% \caption{\stas{this will be edited to show some points on a disc. Maybe projected with colorbar.}}
% \label{fig:gaussian}
% \end{wrapfigure}

Since \citeauthor{HYVARINEN1999429} proved the unidentifiability of nonlinear-ICA, various techniques were introduced to combat the issue both in the context of this model and the VAE that can be framed as its generalization \citep{khemakhem2020variationalautoencodersnonlinearica}.  Common for all of them is the idea to restrict the space of all possible parameters by either limiting the flexibility of the model (e.g. reducing to ICA \cite{ICA_linear}), introducing supervision through auxiliary variables \citep{khemakhem2020variationalautoencodersnonlinearica,mita2021identifiabledoublevaedisentangled}  or collecting more data in a specific way \citep{gresele2019incompleterosettastoneproblem, yao2024multiviewcausalrepresentationlearning}. 

Focusing on the learned latent representations themselves, these works seek to make the model identifiable or reduce the set of its indeterminacy transformations at the cost of limited expressivity, introducing inductive biases through a conditional prior on the latent variables or gathering more data which is not necessarily feasible. 

\textbf{In this paper}, we shift the focus away from the identifiability of the latent representations and instead consider identifiability of a distance measure in the latent space. This idea is motivated by the fact that applications of representation learning in healthcare and science are often in the context of some downstream task on the learned manifold \citep{Detlefsen_2022, Landi_2020}. Thus, achieving identifiability of a distance measure that allows the exploration of the latent space will render the subsequent tasks such as clustering and classification identifiable leading to reliable discoveries.

In particular, we prove that the geodesic distance measure in the latent space of a latent variable model is invariant under all indeterminacy transformation, ie. giving rise to a strongly identifiable metric space without relying on identifiability of the model parameters themselves. Furthermore, we provide an implementation that translates the method into action and showcases the validity of the result in practice. Additional experiments show that geodesic distances exhibit the same invariant behavior even when we relax the model assumption of injectivity of the decoder. Thus, our method provides strong guarantees when needed as well as identifiable-like properties with SOTA architectures.

\textbf{The outline} of the rest of paper starts with Section~\ref{relatedw} where we put our work into perspective with related literature. In Section~\ref{prelim} we will cover the necessary preliminaries covering the basic definitions as well as reintroducing known results in Riemannian geometry and Generative Models literature. Section~\ref{result} will introduce and prove the main result of the paper establishing the identifiability of latent metric spaces, whereas Section 4 will showcase its validity on real data while providing an implementation. Sections 5 and 6 will respectively discus the result and conclude the paper. 



